Novelty Controlled Paraphrase Generation with Retrieval Augmented Conditional Prompt Tuning

Paraphrase generation is a fundamental and long-standing task in natural language processing. In this paper, we concentrate on two contributions to the task: (1) we propose Retrieval Augmented Prompt Tuning (RAPT) as a parameter-efficient method to adapt large pre-trained language models for paraphrase generation; (2) we propose Novelty Conditioned RAPT (NC-RAPT) as a simple model-agnostic method of using specialized prompt tokens for controlled paraphrase generation with varying levels of lexical novelty. By conducting extensive experiments on four datasets, we demonstrate the effectiveness of the proposed approaches for retaining the semantic content of the original text while inducing lexical novelty in the generation.

==> extras.tex <==
\begin{comment}
""
Input: Why do all of my questions get marked as needing improvement

L-PT: Why do my questions get marked as needing improvement

L-RAPT: Why are my questions still being marked as needing improvement

L-RANCoPT [HIGH]: Why is my question being marked as needs to be improved?

L-RANCoPT [LOW]: Why do all of my questions get marked as needing improvement?

Input: Will microsoft’s acquisition of linkedin prove useful for microsoft if so what will useful look like?

L-PT: Will microsoft’s acquisition of linkedin prove useful for microsoft  if so what will useful look like?

L-RAPT: How does microsoft benefit from linkedin acquisition?

L-RANCoPT [HIGH]: How does microsoft benefit from linkedin acquisition?

L-RANCoPT [LOW]: Will microsoft’s acquisition of linkedin prove useful for microsoft if so what will useful look like?
""
\end{comment}
